SIOD: Single Instance Annotated Per Category Per Image for Object Detection

Object detection under imperfect data receives great attention recently. Weakly supervised object detection (WSOD) suffers from severe localization issues due to the lack of instance-level annotation, while semi-supervised object detection (SSOD) remains challenging led by the inter-image discrepancy between labeled and unlabeled data. In this study, we propose the Single Instance annotated Object Detection (SIOD), requiring only one instance annotation for each existing category in an image. Degraded from inter-task (WSOD) or inter-image (SSOD) discrepancies to the intra-image discrepancy, SIOD provides more reliable and rich prior knowledge for mining the rest of unlabeled instances and trades off the annotation cost and performance. Under the SIOD setting, we propose a simple yet effective framework, termed Dual-Mining (DMiner), which consists of a Similarity-based Pseudo Label Generating module (SPLG) and a Pixel-level Group Contrastive Learning module (PGCL). SPLG firstly mines latent instances from feature representation space to alleviate the annotation missing problem. To avoid being misled by inaccurate pseudo labels, we propose PGCL to boost the tolerance to false pseudo labels. Extensive experiments on MS COCO verify the feasibility of the SIOD setting and the superiority of the proposed method, which obtains consistent and significant improvements compared to baseline methods and achieves comparable results with fully supervised object detection (FSOD) methods with only 40% instances annotated.

==> Figures/frcnn_fcos.tex <==
\begin{figure}
\centering

    \includegraphics[width=0.49\linewidth]{Images/pos-neg-vis/frcnn_fcos_a.pdf}
    \includegraphics[width=0.49\linewidth]{Images/pos-neg-vis/frcnn_fcos_b.pdf} \\
    \vspace{-0.5mm}
     \begin{minipage}{0.49\linewidth}
    \centering
    \figtext{(a) Faster RCNN}
    \end{minipage}
    \begin{minipage}{0.49\linewidth}
    \centering
    \figtext{(b) FCOS}
    \end{minipage} \\
    \caption{Under the SIOD setup, illustration of positive and negative samples selected by Faster-RCNN(a) and FCOS(b).}
    \label{fig:frcnn_fcos}
\end{figure}

==> reviews.tex <==
reviewer #1
1. In the proposed Pixel-level Group Contrastive Learning, if the selected group contains the false instances with high similarities. How to avoid the effect of these false labels?
2. Could you prove the effectiveness of the proposed method qualitatively? For example, visualize the assigned pseudo label or the pixel-level group.
3. It would be better to consider the computational cost in your comparisons.
4. The writing requires further polishing, and there are many grammatical errors.
- true match -> a true match in Line 138
- the large amount of -> a large amount of in Line 176
- relative -> relatively in Line 249
- there -> there are in Line 415
- the the -> the in Line 457

reviewer #2
1. writing
- I understand the cosine similarity S is the map with the dimension of K x N. However, in Equation 4, S_{pi} is actually vector with the dimension of 1 x N. With the argmax operator, what is the exact meaning of the two outputs c_n and v? Furthermore, why should v multiply by η?
- Also in Equation 6, f_{k0}^{ci} means the primary positive key of each labeled reference instance f_{q}^{ci}. What is the meaning of f_{k0}^{kz}？
- in Table 3, The module is divided into two categories denoted as PCL and PGCL. What is the PCL? Do you want to talk about SPLG?
2. One of my main concerns is that: With only one labeled instance and the measurement of feature similarity, how to guarantee to detect the instance with much different intra-class feature? such as the one with very different pose compared to the annotated exemplar? Consider the fact in many application cases that the feature difference of intra-class may be greater than that of inter-classes, the reviewer doubt the generalization of the proposed method. In one word, the limitation of the proposed work should be given and discussed in-depth.
3. From the definition of SIOD, I understand the dataset contains the single annotated instance per category per image. However, how to determine the initial annotated instance? In other words, for example in Figure 2, there are several instances of person class in the image. Why is the left person labeled rather than the right one?
4. From what I understand, the annotation form discussed in the manuscript is bounding box, not pixel-level. Therefore, for general object detection, one situation that can arise with high probability is that one gt box contains two samples, especially in crowded scenes. In other words, one gt box is meant to label one object but mislabel other objects at the same time. In this situation, it brings about one problem that from the view of pixel-level, the mislabel objects are actually unlabeled, but the SPLG thinks they are labeled (Line346-350). Will this cause some confusion?
5 How to define the primary positive key f_{k0}^{ci} in Equation 6?

reviewer #3
1. In line 22, It's described more accurately by replacing "for each category in an image" with "for each existing category in an image". This is just advice.
2. The notation is well illustrated in the SPLG module in Fig. 2. Why not the PGCL module?
3. How to get the class prediction in Line 386 on the Right. Does it the same as the heatmap for the SPLG module?
4. CenterNet and FCOS are chosen as a baseline. Both of them are proposed in 2019, two years ago. Why do you use a stronger baseline? For CenterNet in Table 1, how about the result using the backbone hourglass? With CenterNet-Res101, the performance drops more than with CenterNet-Res18. Is there any analysis of why?
5. Even though resnet18 is used as the backbone for Table 2, the training data are still not kept the same. Does the comparison in the Table is truly fair?
6. Some minor issues:
a. The image is masked seriously so that I cannot see what red, green, and blue indicates for what category. As one instance is annotated, I think the different colors stand for different classes.
b. In Eq. 3, why two times L2-norm are used? The first L2-norm is used in Line 399 to normalize feature F and the second is used in Eq. 3.
c. G^t in Line 351 one the Left, G_{c_i} in Eq. 3, and f_{k0}^{c_i} in Line 395 is the same feature for the reference sample. It's better to keep the same so that it's easy to follow.
d. In Eq. 5, using a small font to make the equation in one line is better for the "otherwise".
e. In the right term of Eq. 6, f^{cz}_{k0} --> f^{c_z}_{k0}?
f. PCL--> SPLG in Table 1?
7. Why not choose more recent baseline to show the generalization ability to different one-stage object detector?
8. Pseudo label generationand refinement are two normal ways for incomplete annotation. Pseudo label generation module is straight-farward and the refinement uses the existing approach. It decrease the novelty of the DMiner.
9. The paper gives lots of comparison between the proposed SIODand WSOD, SSOD and SAOD . However, only SSOD and SAOD are compared in Section 4.3. It lacks comparison between WSOD method and SAOD.
10. For the top-m positions in PGCL, a continutional way maybe better than an instance value. Ref: Multiple Anchor Learning for Visual Object Detection, CVPR 2020.
